PoBO: A Polynomial Bounding Method for Chance-Constrained Yield-Aware Optimization of Photonic ICs

Conventional yield optimization algorithms try to maximize the success rate of a circuit under process variations. These methods often obtain a high yield but reach a design performance that is far from the optimal value. This paper investigates an alternative yield-aware optimization for photonic ICs: we will optimize the circuit design performance while ensuring a high yield requirement. This problem was recently formulated as a chance-constrained optimization, and the chance constraint was converted to a stronger constraint with statistical moments. Such a conversion reduces the feasible set and sometimes leads to an over-conservative design. To address this fundamental challenge, this paper proposes a carefully designed polynomial function, called optimal polynomial kinship function, to bound the chance constraint more accurately. We modify existing kinship functions via relaxing the independence and convexity requirements, which fits our more general uncertainty modeling and tightens the bounding functions. The proposed method enables a global optimum search for the design variables via polynomial optimization. We validate this method with a synthetic function and two photonic IC design benchmarks, showing that our method can obtain better design performance while meeting a pre-specified yield requirement. Many other advanced problems of yield-aware optimization and more general safety-critical design/control can be solved based on this work in the future.

==> Others/temp.tex <==
\section{Introduction}
\label{introduction}
The increasing process variations have resulted in significant performance degradation and yield loss~\cite{gielen2008emerging,chen2013process,lu2017performance}. 
Therefore, there has been a long history of investigating yield optimization and yield-aware robust design in the electronic \hzc{and photonic} design automation (EDA \hzc{and PDA}) community.

%%%%%%%%%%%%%%%%%%%%%
The geometric yield optimization methods~\cite{antreich1994circuit} aimed to optimize the worst-case performance under process variations.
A yield-aware Pareto surface was adopted for hierarchical circuit design space exploration~\cite{tiwary2006generation}.
A gradient-based yield optimization leveraging the stochastic sensitivity of yield with respect to design parameters was proposed in~\cite{gong2012fast}.
Bayesian yield optimization~\cite{wang2017efficient} aimed to maximize the posterior probability of design parameters under the conditions that the yield constraints are satisfied. 
Other yield-aware design techniques include yield-driven iterative robust design~\cite{li2009yield}, geometric programming-based approaches~\cite{xu2009regular}, geostatistics-motivated performance modeling~\cite{yu2007yield}, computational intelligence assisted approaches~\cite{liu2011efficient}, corner-based method~\cite{barros2010analog}, and so forth.
%Hierarchical approaches have also been proposed for system-level yield optimization~\cite{yu2008yield}.
%\zz{Need much more references. For instance, Xin Li's group, Lei He's group and Rob Rutenbar's group have done lots of work on yield optimization.} 

Yield estimation is the key component in a yield optimizer~\cite{gong2014variability,li2012efficient}. 
Advanced yield estimators can be generally classified as Monte-Carlo-based~\cite{singhee2008practical,papoulis2001probability} and non-Monte-Carlo-based~\cite{gu2008efficient,gong2012fast,9428031} methods. Among the non-Monte-Carlo ones, surrogate modeling aims to approximate some circuit behaviors under variations to speed up the sampling and simulation process~\cite{shi2019meta,yao2014efficient,li2006asymptotic}. 
%In order to accelerate yield estimator and optimizer, various surrogate models can be constructed to speed up the sampling and simulation process~\cite{shi2019meta,yao2014efficient}. 
Typical surrogate models include posynomial models~\cite{li2004robust}, linear quadratic models~\cite{li2008quadratic}, support vector machine~\cite{ciccazzo2015svm}, Gaussian process~\cite{sanabria2020gaussian,wang2017yield}, sparse polynomial~\cite{wang2014enabling}, generalized polynomial chaos expansions~\cite{xiu2003modeling,zhang2013stochastic}, and some variants~\cite{trinchero2020combining}. 
\hzc{Focusing on generalized polynomial chaos expansion,} advanced techniques have also been developed to handle high-dimensional~\cite{li2010finding,zhang2014enabling,zhang2016big,He2020EPEPS,he2021high}, mixed-integer~\cite{He2019ICCAD} or non-Gaussian correlated~\cite{cui2018stochastic} process variations. \hzc{They have also been widely used in robust IC design~\cite{waqas2018stochastic,weng2017stochastic}.}

%%%%%%%%%%%%%%%%%%%%%
While most existing yield optimization approaches try to maximize the yield of a circuit, the obtained design performance (e.g., signal gain, power dissipation) may be far from the achievable optimal solution. Recently, an alternative approach was proposed in~\cite{cui2020chance} to achieve both excellent yield and design performance. Instead of simply maximizing the yield, the work~\cite{cui2020chance} optimizes a design performance metric while enforcing a high yield requirement. Specifically, the yield requirement is formulated as some chance constraints~\cite{shapiro2014lectures}, which are further transformed to tractable constraints of the first and second statistical moments. 
\hzc{The chance constrained modeling has been widely used in many engineering fields~\cite{mesbah2014stochastic,vitus2015stochastic,wang2017chance}.}
The moment method offers a provably sufficient condition of the chance constraint. However, the bounding gap may be too large in many applications~\cite{van2016generalized}.
%However, the moment constraints is a provably sufficient condition of the chance-constrained, but may be over-tight in many applications~\cite{van2016generalized}.
The resulting overly-reduced feasible region may lead to an over-conservative design. 

\textbf{Paper contributions.}
This paper proposes a novel \textbf{Po}lynomial \textbf{B}ounding method for chance-constrained yield-aware \textbf{O}ptimization (PoBO) under truncated non-Gaussian correlated variations. Leveraging the recent uncertainty quantification techniques~\cite{cui2018stochastic,cui2020chance}, PoBO 
employs and modifies the idea of kinship functions~\cite{feng2010kinship} to approximate the original chance constraints with a better polynomial bounding method. PoBO provides a less conservative design than moment-based bounding methods~\cite{cui2020chance} while ensuring a pre-specified yield requirement. 
%The truncated non-Gaussian correlation assumption of the variations is more realistic. It also enables the proposed polynomial relaxation method. 
The specific contributions of this paper include:
\begin{itemize}[leftmargin=*]
    \item A better bounding method of the chance constraints via optimal polynomial kinship functions. Compared with existing work in the control community~\cite{feng2010kinship}, we avoid the assumption of the independence among random variables and the convexity of kinship functions. \hzc{The relaxation allows more general non-Gaussian correlated uncertainty modeling and tightens the bounding functions.}
    \hzc{Within a family of polynomial functions, the optimal polynomial kinship functions can be efficiently solved via semidefinite programming.}
    Our bounding method preserves the polynomial formulation of the provided surrogate models. \hzc{It enables the advanced polynomial optimization solvers, which provide a sequence of convex relaxations via semidefinite optimization and searches for the global design.} 
    %\hzc{Add more detailed introduction}
    \item Numerical implementation of the PoBO framework. Based on available uncertainty quantification solvers, we implement PoBO efficiently based on some pre-calculated optimal polynomial kinship functions and quadrature samples and weights without requiring any additional circuit simulations.
    \item Validations on a synthetic function and two photonic IC design examples. Our method offers better design performance while meeting the pre-specified yield requirements. This method requires a small number of circuit simulations due to its compatibility with recent data-efficient uncertainty quantification methods~\cite{zhang2016big,cui2018stochastic}.
\end{itemize}

While this work focuses on the fundamental theory, algorithms and their validation on small-size photonic circuits, the proposed method can be combined with sparse or low-rank surrogate modeling methods~\cite{li2010finding,zhang2016big} to handle large-scale design cases with much more process variations.

% polynomial reference
%wang2016re, wang2014enabling

